New tools for network time series with an application to COVID-19 hospitalisations

Network time series are becoming increasingly important across many areas in science and medicine and are often characterised by a known or inferred underlying network structure, which can be exploited to make sense of dynamic phenomena that are often high-dimensional. For example, the Generalised Network Autoregressive (GNAR) models exploit such structure parsimoniously. We use the GNAR framework to introduce two association measures: the network and partial network autocorrelation functions, and introduce Corbit (correlation-orbit) plots for visualisation. As with regular autocorrelation plots, Corbit plots permit interpretation of underlying correlation structures and, crucially, aid model selection more rapidly than using other tools such as AIC or BIC. We additionally interpret GNAR processes as generalised graphical models, which constrain the processes' autoregressive structure and exhibit interesting theoretical connections to graphical models via utilization of higher-order interactions. We demonstrate how incorporation of prior information is related to performing variable selection and shrinkage in the GNAR context. We illustrate the usefulness of the GNAR formulation, network autocorrelations and Corbit plots by modelling a COVID-19 network time series of the number of admissions to mechanical ventilation beds at 140 NHS Trusts in England & Wales. We introduce the Wagner plot that can analyse correlations over different time periods or with respect to external covariates. In addition, we introduce plots that quantify the relevance and influence of individual nodes. Our modelling provides insight on the underlying dynamics of the COVID-19 series, highlights two groups of geographically co-located `influential' NHS Trusts and demonstrates superior prediction abilities when compared to existing techniques.

==> gnar_pop_sparse_proof.tex <==
\section*{Proof of Theorem \ref{th: pop_sparsity gnar}}
Assume that $\boldsymbol{X}_t$ is a stationary $\GNAR(p, [s_1, \cdots, s_p])$ process for which the underlying network structure $\mathcal{G} = (\mathcal{K}, \mathcal{E})$ is static and with full rank spectral matrix. Throughout this section the following notation and definitions are used 
\begin{itemize} \label{def: notation and sets}
    \item $\boldsymbol{X}_t$ multivariate time series.
    \item $r^* = \max(s_1, s_2, \cdots, s_p)$ the maximum $\rstage$ active depth.
    \item $\cup_{r = 1}^{r^*} \mathcal{N}_{r} (i) =: \mathcal{N} (i)$ the set of active $\rstage$ neighbors with respect to node $i$.
    \item $\mathcal{A}_r := (i, j) \in \mathcal{A}_r \iff \exists l \in \mathcal{K}$ such that $d(i, l) \leq r$ and $d(l, j) \leq r;$ 
    the set of active $\rstage$ pairs in neighborhood regressions.
    \item $\mathcal{P}_{r} := \mathcal{A}_{r} - \mathcal{A}_{r - 1}$ the set of pairs which activate exactly at a distance equal to $r$ 
    \newline (i.e., $(i, j) \in \mathcal{P}_r \iff \exists l \in \mathcal{K}$ such that $d(i, l) \leq r$, $d(l, j) \leq r$ and $(i, j) \notin \mathcal{A}_{r - 1}$).
    \item $\bmat{f}(\omega)$ spectral matrix of $\boldsymbol{X}_t$.
    \item $\bmat{S}(\omega) = \{\bmat{f}(\omega)\}^{-1}$ inverse spectral matrix of $\boldsymbol{X}_t$. 
    \item $f(\cdot) \equiv 0$ the function $f$ is identically zero in its domain.
    \item $f_{i, j | \mathcal{A}^{(ij)}}(\omega)$ conditional cross-spectrum between $X_{i, t}$ and $X_{j, t}$.
    \item $X_{i, t} \perp X_{j, t + h} | \mathcal{A}^{(ij)}$ the two time series are independent given all the other ones in $\mathcal{A}^{(ij)}$.
    \item $\{\bmat{S}_{\mathcal{A}^{(ij)}} (\omega) \}$ inverse spectral matrix constrained to the set $\mathcal{A}^{(ij)}$.
    \item $ \boldsymbol{f}_{i, \mathcal{A}^{(ij)}} (\omega)$ $i$th column of the spectral matrix without the $i$th entry.
\end{itemize}
%Proof starts here
\newpage
\begin{proposition} \label{prop: distance for conditional independence}
    Assume that $\boldsymbol{X}_t$ is a stationary $\GNAR(p, [s_1, \cdots, s_p])$ process for which the underlying network structure $\mathcal{G} = (\mathcal{K}, \mathcal{E})$ is static and with the same notation as above, then $(i, j) \notin \mathcal{A}_{r^*}$ if and only if $d(i, j) \geq 2 r^* + 1$. And, that $(i, j) \in \mathcal{P}_{r^*}$ if and only if $d(i, j) \in \{2 r^* - 1, 2 r^* \}$.
\end{proposition}
\begin{proof}
    Let $(i, j) \notin \mathcal{A}_{r^*}$, then there does not exist $l \in \mathcal{K}$ such that
    \begin{equation} \label{eq: borough active set condition}
        d(i,l) \leq r^* \textit{ and  } d(j, l) \leq r^* .
    \end{equation}
    Using (\ref{eq: borough active set condition}) note that if there is at least one $l \in  \mathcal{N} (i) \cap  \mathcal{N} (j)$, then such $l$ satisfies $d(i, l) \leq r^*$ and $d(j, l) \leq r^*$, and by definition we have that $(i, j) \in \mathcal{A}_{r^*}$, thus, $(i, j) \notin \mathcal{A}_{r^*}$ if and only if $\mathcal{N} (i) \cap  \mathcal{N} (j) = \varnothing$.
    \par
    Now, suppose that $d(i, j) \leq 2 r^*$, then we can choose $l$ such that 
        $d(i, l) = r$,
    for some $r \in \{1, \cdots, r^* \}$, hence, $l \in \mathcal{N} (i)$. Note that since $d(i, j) > r^*$, we can write
    \begin{align*}
        d(i, j) &= d(i, l) + d(j, l) \\
        &= r + d(j, l) \leq 2 r^* \\
        &\iff d(j, l) \leq r^*,
    \end{align*}
    so we have that $l \in \mathcal{N} (j)$, and 
    \begin{equation*}
        l \in  \mathcal{N} (i) \cap  \mathcal{N} (j) \dagger
    \end{equation*}
    a contradiction since $(i, j) \notin \mathcal{A}_{r^*}$, therefore, 
        $d(i, j) \geq 2 r^* + 1$.
    Now, decrease $r^*$ to $(r^* -1)$, since $(i, j) \notin \mathcal{A}_{r^* - 1}$ if and only if $d(i, j) \geq 2 r^* - 1$, we have that $\mathcal{A}_{r^* - 1} \subseteq \mathcal{A}_{r^*}$, and 
    $$2 r^* - 1 \leq d(i, j) < 2 r^* + 1 \iff (i, j) \in \mathcal{A}_{r^*} - \mathcal{A}_{r^* - 1},$$
    hence, $(i, j) \in \mathcal{P}_{r^*}$ if and only if $d(i, j) \in \{2 r^* - 1, 2 r^* \}$.
\end{proof}
\newpage
Recall from time series analysis that the best linear predictor up to a certain lag restricted to a subset of active nodes $\mathcal{A} \subseteq \mathcal{K}$ solves for the optimal linear filter with respect to mean squared error. Set $\mathcal{A}^{(ij)} := \mathcal{K} - \{i, j\}$, then the error of the optimal filter conditioning on $\mathcal{A}^{(ij)}$ is given by

\begin{equation} \label{eq: opt filter}
   u_{i, t}^{(ij)} := u_{i, t | \mathcal{A}^{(ij)} } = X_{i, t} - a_{i} - \sum_{k = 1}^{p} \sum_{l \in \mathcal{A}_{r^*}^{(j)}} 
   \gamma_{k}^{il} X_{l, t - k},
\end{equation}
where $\mathcal{A}_{r^*}^{(j)} = \mathcal{A}^{(ij)} \cap \mathcal{N} (i)$  and $a_i$ is the optimal mean constant; see \cite{brockwell_davis}. 
Following \cite{graph_series}, define the conditional dependence structure based on the cross-spectrum between the conditional time series $X_{i, t} | \mathcal{A}^{(ij)}$ and $X_{j, t} | \mathcal{A}^{(ij)}$ by noting that these two time series are uncorrelated at all lags if and only if the conditional cross-spectrum $f_{i, j | \mathcal{A}^{(ij)}}(\omega)$ is identically zero for all frequencies $\omega \in [-\pi, \pi]$. We will make use of the following result proved in \cite{graph_series}.
\begin{theorem}{[\cite{graph_series}]} \label{th: inv spec cross indentity}
Let $\boldsymbol{X}_t$ be a stationary multivariate time series, if the spectral matrix $\bmat{f}(\omega)$ has full rank, then
\begin{align*}
    f_{i, j | \mathcal{A}^{(ij)}}(\omega) &:= f_{u_{i}^{(ij)} u_{j}^{(ij)}} (\omega), \\
    f_{i, j | \mathcal{A}^{(ij)}}(\omega) &= - [\bmat{S} (\omega)]_{ij}.
\end{align*}
\end{theorem}
The relevance of Theorem \ref{th: inv spec cross indentity} is that it enables us to identify conditional independence by looking at the inverse spectral matrix $\bmat{S} (\omega)$, rather than by computing all possible conditional cross-spectrum values. Hence, the inverse spectral matrix is related to multivariate time series models as the concentration (inverse-covariance) matrix is to Gaussian Graphical Models; see \cite{graph_lasso}. 
This allows to state results from \cite{graph_series} and \cite{brillinger} in the following Lemma. 
\newpage
\begin{lemma}{[\cite{graph_series}, and \cite{brillinger} ]} \label{lma: conditional equivalences}
Let $\boldsymbol{X}_{t} \in \mathbb{R}^d$ be a stationary multivariate process, with the same notation as above, then 
\begin{align} \label{eq: conditional independence equivalence}
    X_{i, t} \perp X_{j, t + h} | \mathcal{A}^{(ij)} \textit{ for all } h  &\iff \cov (u_{i, t}^{(ij)}, u_{j, t + h}^{(ij)} ) \equiv 0, \nonumber \\
    &\iff f_{i, j | \mathcal{A}^{(ij)}}(\omega) \equiv 0, \nonumber \\
    &\iff [\bmat{f}(\omega)]_{ij} - \boldsymbol{f}_{i, \mathcal{A}^{(ij)}} (\omega) \{ \bmat{S}_{\mathcal{A}^{(ij)}} (\omega) \}^{-1}  
    \boldsymbol{f}_{\mathcal{A}^{(ij)}, j} (\omega), \nonumber \\
    &\iff [\bmat{S} (\omega)]_{ij} \equiv 0.
\end{align}
\end{lemma}
A partial correlation graph satisfies the Markov properties if we define the absence of an edge as the relation $ X_{i, t} \perp X_{j, t + h} | \mathcal{A}^{(ij)} \textit{ at all } h$, which makes explicit the relationship between nodes $i$ and $j$ (i.e., $i$ and $j$ are uncorrelated at all lags given all the other nodes in the graph); see \cite{graph_series}. GNAR generalizes this idea by noting that the conditional independence can be extracted from paths in the graph rather than just from existing edges. 

\begin{definition} \label{def: conditional indep definition}
Let $\boldsymbol{X}_t$ be a stationary multivariate process with an underlying $\GNAR$ structure $\mathcal{G} = (\mathcal{K}, \mathcal{E})$, the $\GNAR$ generalized correlation graph $G = (\mathcal{K}, E)$ is an undirected graph which satisfies $d_{E} (i, j) > r^*$ if and only if nodes $i$ and $j$ are independent given all the other nodes, which we write as
\begin{equation*}
     X_{i, t} \perp X_{j, t + h} | \mathcal{A}^{(ij)} \textit{ at all } h \iff d_{E} (i, j) > r^*.
\end{equation*}
Furthermore, the strength of dependence can be recovered from $G$ in the sense that if $d_{E} (i, j) = r$ for some $r \in \{1, \cdots, r^* \}$, then constraining the $\GNAR$ model to maximum $\rstage$ depth of $(r - 1)$ will uncorrelate the two nodal time series (i.e., $ X_{i, t} \perp X_{j, t + h}$ at all lags $h$).
\end{definition}
\newpage
Intuitively, Definition \ref{def: conditional indep definition} proposes that two nodes in the underlying network $\mathcal{G}$ are conditionally independent if and only if the shortest path between their active $\rstage$ neighbors has a length of at least one (i.e., they do not have common active $\rstage$ neighbors). This condition expresses mathematically that no active projection path is long enough to contain both $i$ and $j$.
\par
Before continuing we mention the following result from \cite{graph_series}. 
\begin{proposition}{[\cite{graph_series}]} \label{prop: conditional residual}
Let $\boldsymbol{X}_t$ be a multivariate time series with correlation structure given by $\mathcal{G} = (\mathcal{K}, \mathcal{E})$ and spectral matrix $\bmat{f}(\omega)$ which has full rank for all frequencies $\omega \in [-\pi, \pi]$, then
    $$    (i, j) \notin \mathcal{E}  \iff [\bmat{S}(\omega)]_{ij} \equiv 0.
    $$
\end{proposition}
The following proposition is necessary as well.
\begin{proposition} \label{prop: var constrains}
Let $\boldsymbol{X}_t$ be a stationary $\GNAR$ process with full rank spectral matrix $\bmat{f} (\omega)$, static underlying network $\mathcal{G} = (\mathcal{K}, \mathcal{E})$ structure and maximum active $\rstage$ neighborhood regression $r^*$, then we have that
\begin{equation*}
    (i, j) \notin \mathcal{A}_{r^*} \textit{ if and only if } X_{i, t} \perp X_{j, t + h} | \mathcal{A}^{(ij)} \textit{ at all lags } h.
\end{equation*}
\end{proposition}
\begin{proof}
Recall the VAR representation of  $\GNAR(p, [s_1, \cdots, s_p])$ process given by (\ref{eq: sparse var}),
\begin{equation*}
    X_{i, t} = \sum_{k = 1}^{p} \big( \phi_{k}^{ii} X_{i , t- k} + \underset{j \in \mathcal{N} (i)}{\sum} \phi_{k}^{ij} X_{j , t- k}
    \big )+ u_{i, t},
\end{equation*}
for which the autoregressive matrices are given by 
$$\bmat{\Phi}_k = \{\diag(\alpha_{ik}) + \sum_{r = 1}^{s_k} \beta_{kr} (\bmat{W} \odot \bmat{S}_r ) \},$$
and the entries satisfy
\begin{equation*}
    [\bmat{\Phi}_k]_{ij} = \alpha_{ik} \mathbb{I}(i = j) + \beta_{k r} w_{i j} \mathbb{I}(i \neq j),
\end{equation*}
\newpage
moreover, since $\phi_{k}^{ij} = \beta_{kr} w_{ij}$ and $\phi_{k}^{ji} = \beta_{kr} w_{ji}$ we have that
\begin{equation} \label{eq: ar coeffss equiv}
    \phi_{k}^{ij} \equiv 0 \iff \beta_{kr} \equiv 0 \iff \phi_{k}^{ji} \equiv 0,
\end{equation}
regardless of the connection weights between nodes, it is active $\rstage$ depth which activates a connection between two nodes. And that the characteristic matrix polynomial for $z \in \mathbb{C}$ is given by
$$ \bmat{\Phi}(z) := \bmat{I_d} - \sum_{k = 1}^{p} \bmat{\Phi}_k z^k, $$
and recall that $\bmat{S} (\omega)$ satisfies; see \cite{brockwell_davis},
\begin{equation} \label{eq: inverse spec coeffs}
    \bmat{S} (\omega) = \frac{2 \pi}{\sigma^2} \{\bmat{\Phi}(e^{\imath \omega})\}^T \bmat{\Phi}(e^{-\imath \omega}).
\end{equation}
Now combine (\ref{eq: inverse spec coeffs}) and (\ref{eq: ar coeffss equiv}), so we have that
\begin{equation*}
    [\bmat{S} (\omega)]_{ij} = \frac{2 \pi}{\sigma^2} \sum_{l = 1}^{d} [\{\bmat{\Phi}(e^{\imath \omega})\}^T]_{il} [\bmat{\Phi}(e^{-\imath \omega})]_{lj},
\end{equation*}
hence, we also have that
\begin{equation} \label{eq: inv spec and ar coefs}
    [\bmat{S} (\omega)]_{ij} \equiv 0 \iff  \sum_{l = 1}^{d} [\{\bmat{\Phi}(e^{\imath \omega})\}^T]_{il} [\bmat{\Phi}(e^{-\imath \omega})]_{lj} \equiv 0.
\end{equation}
Assume that $[\{\bmat{\Phi}(e^{\imath \omega})\}^T]_{il} [\bmat{\Phi}(e^{-\imath \omega})]_{lj} \equiv 0$, then the sum in the right hand side of (\ref{eq: inv spec and ar coefs}) is equal to zero, and by combining Lemma \ref{lma: conditional equivalences} and (\ref{eq: inv spec and ar coefs}) we have that
\begin{align} \label{eq: inactive to condtitional independende}
    [\{\bmat{\Phi}(e^{\imath \omega})\}^T]_{il} [\bmat{\Phi}(e^{-\imath \omega})]_{lj} \equiv 0 &\implies  [\bmat{S} (\omega)]_{ij} \equiv 0, \nonumber \\
    &\iff X_{i, t} \perp X_{j, t + h} | \mathcal{A}^{(ij)} \textit{ at all lags } h.
\end{align}
Now, suppose that $(i, j) \notin \mathcal{A}_{r^*}$, then $d(i, j) > r^*$ and there does not exist $l \in \mathcal{K}$ such that $d(i, l) \leq r^*$ and 
$d(j, l) \leq r^*$, where the distances are computed on the underlying network $\mathcal{G}$. 
\newpage
Thus, for all $l \in \mathcal{A}^{(ij)}$ we have that
\begin{align*} \label{eq: first prop cond independence}
    d(i, l) \leq r^* &\implies d(j, l) > r^*, \nonumber \\
    &\implies \phi_{k}^{lj} \equiv 0,
\end{align*}
then since $l$ and $j$, using the above and (\ref{eq: ar coeffss equiv}), do not influence each other we have that
\begin{equation*}
    [\bmat{\Phi}(e^{-\imath \omega})]_{lj} \equiv 0 \implies [\{\bmat{\Phi}(e^{\imath \omega})\}^T]_{il} [\bmat{\Phi}(e^{-\imath \omega})]_{lj} \equiv 0.
\end{equation*}
Note that the argument above holds similarly if $ d(j, l) \leq r^*$, and that if $d(i, l) > r^*$ and $d(j, l) > r^*$, then we have that 
$\phi_{k}^{lj} \equiv 0 \equiv \phi_{k}^{li},$
so by (\ref{eq: inactive to condtitional independende}) and the arguments above we have that
\begin{equation}  \label{eq: first prop cond independence end}
    (i, j) \notin \mathcal{A}_{r^*} \implies X_{i, t} \perp X_{j, t + h} | \mathcal{A}^{(ij)} \textit{ at all lags } h.
\end{equation}
We proceed to prove the other direction, assume that $(i, j) \in \mathcal{A}_{r^*}$, then there exists at least one other nodal time series such that its corresponding node $l \in \mathcal{K}$, $d(i, l) \leq r^*$ and  $d(j, l) \leq r^*$. Hence, by (\ref{eq: inv spec and ar coefs}, \ref{eq: inverse spec coeffs}, \ref{eq: ar coeffss equiv}) we have that 
\begin{equation*}
    (i, j) \in \mathcal{A}_{r^*} \implies  [\bmat{S} (\omega)]_{ij} \not\equiv 0,
\end{equation*}
which by Lemma \ref{lma: conditional equivalences} gives
\begin{equation} \label{eq: second prop cond independence end}
     (i, j) \in \mathcal{A}_{r^*} \implies X_{i, t} \not\perp X_{j, t + h} | \mathcal{A}^{(ij)} \textit{ at all lags } h.
\end{equation}
Finally, combining (\ref{eq: first prop cond independence end}, \ref{eq: second prop cond independence end}) finishes the proof.
\end{proof}
\newpage
Now it is possible to prove Theorem \ref{th: pop_sparsity gnar}, we start by proving the first part (i.e., $a$).
\begin{proof}
Consider the stationary GNAR process $\boldsymbol{X}_t$, we can embed a latent graphical process $\tilde{\boldsymbol{X}}_t$ to this GNAR process by connecting all nodes which fail to satisfy 
\newline $X_{i, t} \perp X_{j, t + h} | \mathcal{A}^{(ij)} \textit{ at all lags } h$. And, 
%And, note that the optimal filters given by (\ref{eq: opt filter}) are uncorrelated at all lags $h$ if and only if nodes $i$ and $j$ do not collide in an active projection path, then 
that by Lemma \ref{lma: conditional equivalences} and Theorem \ref{th: inv spec cross indentity} we have that 
\begin{equation} \label{eq: path length equivalence}
    X_{i, t} \perp X_{j, t + h} | \mathcal{A}^{(ij)} \textit{ for all } h \iff [\bmat{S}(\omega)]_{ij} \equiv 0 .
\end{equation}

Now, denote by $\tilde{\mathcal{G}} = (\mathcal{K}, \tilde{\mathcal{E}})$ the corresponding partial correlation graph. And, connecting (\ref{eq: path length equivalence}), Theorem \ref{th: inv spec cross indentity} and Proposition \ref{prop: conditional residual} we have that 
\begin{align} \label{eq: end first part}
     (i, j) \notin \tilde{\mathcal{E}} &\iff  [\bmat{S}(\omega)]_{ij} \equiv 0 \nonumber \\
     &\iff X_{i, t} \perp X_{j, t + h} | \mathcal{A}^{(ij)} \textit{ at all } h \nonumber \\
     &\iff \cov (u_{i, t}^{(ij)}, u_{j, t + h}^{(ij)} ) \equiv 0,
\end{align}
Then by Proposition \ref{prop: var constrains} and (\ref{eq: end first part}) we have that
\begin{equation*}
      (i, j) \notin \tilde{\mathcal{E}} \iff (i, j) \notin \mathcal{A}_{r^*},
\end{equation*}
and by Proposition \ref{prop: distance for conditional independence}, we have that
\begin{equation*}
     (i, j) \notin \tilde{\mathcal{E}} \iff d(i, j) \geq 2 r^* + 1,    
\end{equation*}
which establishes the first part of Theorem \ref{th: pop_sparsity gnar}.
\end{proof}

Before proving the second part we mention the following notions, and recall that our underlying motivation and assumption is that the larger $r$ is the weaker the dependence between $\rstage$ neighbors is. First, we introduce the complex soft-threshold operator.
\newpage
\begin{definition} \label{def: complex sft-thrsh}
    The complex soft-threshold operator is given by
    \begin{align} \label{eq: cmplx sft}
        \sft(z; \rho) : \mathbb{C} &\rightarrow \mathbb{C} \nonumber \\
        z &\mapsto (|z| - \rho)_{+} e^{\imath \phi},
    \end{align}
    where $\phi = \arg(z) \in [0, 2 \pi]$, $\rho \geq 0$, $\imath$ denotes the imaginary unit (i.e., $\imath^2 = -1$), $(\cdot)_{+}$ denotes the positive part operator, and recall that $|z| e^{\imath \phi} = z$. 
\end{definition}
Note that if the argument $\phi \in \{0, \pi \}$, then $\sft(z; \rho)$ recovers the real-valued soft-threshold operator.
Next, we state a mathematical form of distinguishing between different degrees of relevance between nodes. Motivated by distance as a measure of dissimilarity, assume that there exists a cross-correlation hierarchy and define $\rstage$ neighborhood inclusion, with maximum active stage $r^*$, as follows.
\begin{definition} \label{def: rstage hierarchy}
    Let $\boldsymbol{X}_t$ be a stationary $\GNAR$ process with static underlying structure $\mathcal{G} = (\mathcal{K}, \mathcal{E})$ and conditional cross-correlation hierarchy 
    $0 < \tau^{(r^*)}_h < \cdots < \tau^{(r)}_h < \tau^{(r - 1)}_h < \cdots < \tau^{(1)}_h$, then  $(i, j) \in \mathcal{A}_r \textit{ if and only if }$ the following conditions hold
    \begin{align*}
      \sft (| \cov (u_{i, t}^{(ij)}, u_{j, t + h}^{(ij)} )|;  \tau^{(r - 1)}_h) &\equiv 0, \\
      \sft (| \cov (u_{i, t}^{(ij)}, u_{j, t + h}^{(ij)} )|;  \tau^{(r)}_h) &\not\equiv 0.
    \end{align*}
\end{definition}
Definition \ref{def: rstage hierarchy} makes explicit our assumption that the further nodes are in the graph, the less dependent they are. It enables us to reparameterize a GNAR process by punching out weak dependencies just by decreasing the length of maximum $\rstage$ neighborhood regression (i.e., if we increase the conditional cross-correlation threshold, then nodes further from each other become conditionally independent). 
\newpage
A possible way of interpreting Definition \ref{def: rstage hierarchy} is that it makes explicit the idea of a correlation index by distinguishing between different thresholds $\tau^{(r)}_h$ of relevance for which the underlying GNAR structure $\mathcal{G}$ captures the different strengths.
\par
A useful consequence of Definition \ref{def: rstage hierarchy} is that if the cross-correlation hierarchy exists, then by Theorem \ref{th: inv spec cross indentity} there exists a cross-spectrum hierarchy 
$\infty > \rho^{(1)} >  \rho^{(2)} > \cdots > \rho^{(r^*)} >  \rho^{(r^* + 1)} = 0 $ such that
\begin{equation*}
    \tau^{(r)}_h \leq |\cov (u_{i, t}^{(ij)}, u_{j, t + h}^{(ij)} )| < \tau^{(r - 1)}_h \iff 
     \rho^{(r)} \leq |[\bmat{S}(\omega)]_{ij}| < \rho^{(r - 1)},
\end{equation*}
for all $h$ and at all $\omega \in [-\pi, \pi]$, thus, defining $\rstage$ neighborhood inclusion as in Definition \ref{def: rstage hierarchy} guarantees the existence of a cross-spectrum hierarchy.
\par
Now, it is possible to define an $\rstage$ sequence of inverse spectral matrices as
\begin{equation} \label{eq: r stage inv matrix}
    \bmat{S}^{(r)}(\omega) := \sft \big( \bmat{S} (\omega) + \rho^{(r)} \diag\{e^{\imath \phi_{ii}}\};  \rho^{(r)} \big),
\end{equation}
where $\phi_{ii}$ is the argument of the diagonal entries in $\bmat{S} (\omega)$ and $\sft(z; \rho)$ is applied entry-wise to $\bmat{S} (\omega)$. Note that the diagonal of $\bmat{S} (\omega)$ does not change for any $r \in \{1, \cdots, r^*\}$.
And, that the sequence satisfies 
$$\normx{\bmat{S}(\omega) }_0 < \normx{\bmat{S}^{(r)}(\omega) }_0,$$ 
for all active $r$, and since $\rho^{(r + 1)} < \rho^{(r)}$, also
$$\normx{\bmat{S}^{(r + 1)}(\omega) }_0 \leq \normx{\bmat{S}^{(r)}(\omega) }_0,$$
where $\normx{ \cdot }_0$ counts the number of non-zero entries in the matrix. The sequence above makes explicit the different strengths of dependence between nodes, as $r$ decreases the $\bmat{S}^{(r)}(\omega)$ become sparser which results in a model with fewer nodes influencing each other; see Section \ref{sec: graph model connection}.
\newpage
We are ready to prove the second part (i.e., $b$) of Theorem \ref{th: pop_sparsity gnar}.
\begin{proof}
Assume that $\bmat{f} (\omega)$ has full rank and that the sequence of $\{\bmat{S}^{(r)} (\omega) \}$ are non-singular. Define the sequence of partial correlation graphs 
$\mathcal{G}^{(r)} = (\mathcal{K}, \mathcal{E}^{(r)})$ as the one which satisfies $(i, j) \notin \mathcal{E}^{(r)}$ if and only if $X_{i, t} \perp X_{j, t + h} | \mathcal{A}^{(ij)}$ at all lags $h$ when constraining $\rstage$ depth to $r \in \{1, \cdots, r^*\}$.
By Theorem \ref{th: inv spec cross indentity} and Proposition \ref{prop: var constrains}
we have that
\begin{equation} \label{eq: r sequence equivalence}
    (i, j) \notin \mathcal{E}^{(r)}  \iff [\bmat{S}^{(r)}(\omega)]_{ij} \equiv 0, 
\end{equation}
Using (\ref{eq: r sequence equivalence}) we have that the sequence of edge sets satisfies
\begin{equation} \label{eq: edge set sequence}
     \mathcal{E}^{(1)} \subset \cdots \subset \mathcal{E}^{(r)} \subset \mathcal{E}^{(r + 1)} \subset \cdots  \subset \tilde{\mathcal{E}},
\end{equation}
where $\tilde{\mathcal{E}}$ is defined as in (\ref{eq: end first part}). Note that once a pair of edges become conditionally independent they stay so since the soft-threshold operator maps that entry to zero for all larger $\rho^{(r)}$ in the cross-spectrum hierarchy, this idea allows us to prune the underlying graph by removing edges based on the strength (i.e., magnitude) of the conditional cross-spectrum $f_{i, j | \mathcal{A}^{(ij)}}(\omega)$; see Lemma \ref{lma: conditional equivalences}. Now consider a pair of nodes $i$ and $j$ which satisfy
\begin{equation} \label{eq: second part heart}
    \rho^{(r)} \leq |[\bmat{S}(\omega)]_{ij}| < \rho^{(r - 1)},
\end{equation}
for all $\omega \in [-\pi, \pi]$, then, applying the soft-threshold given by Definition \ref{def: complex sft-thrsh} and (\ref{eq: cmplx sft}, \ref{eq: r sequence equivalence}) to this pair results in 
$(i, j) \in \mathcal{E}^{(r)}$, and $(i, j) \notin \mathcal{E}^{(r - 1)}$, thus, we have that 
\begin{align} \label{eq: second part inv equivalences}
    &(\ref{eq: second part heart}) \implies (i, j) \in \mathcal{E}^{(r)} - \mathcal{E}^{(r - 1)}, \nonumber \\
    &(i, j) \in \mathcal{E}^{(1)} \implies (i, j) \in \bigcap_{r = r^*}^{1} \mathcal{E}^{(r)}, \nonumber \\
    &(i, j) \in \mathcal{E}^{(r)} \implies (i, j) \in \bigcap_{s = r^*}^{r} \mathcal{E}^{(s)} .
\end{align}
\newpage
Following the ideas above, consider the graph $\mathcal{G}^{(1)} = (\mathcal{K}, \mathcal{E}^{(1)})$ associated to the strongest connections with edge set $\mathcal{E}^{(1)}$, which is the one with the strongest dependence between nodes as proposed in Definition \ref{def: rstage hierarchy}. 
\par
Using (\ref{eq: second part heart}, \ref{eq: second part inv equivalences}) we have that if $(i, j) \in \mathcal{E}^{(1)}$, then $i$ and $j$ are connected throughout the whole sequence in (\ref{eq: edge set sequence}), and that the edge set sequence satisfies
\begin{align} \label{eq: second part inverse end}
    \mathcal{A}_{1} &= \mathcal{E}^{(1)}, \nonumber \\
    \mathcal{A}_{2} - \mathcal{A}_{1} &= \mathcal{E}^{(2)} - \mathcal{E}^{(1)}, \nonumber \\
    &\cdot \nonumber \\
    \mathcal{A}_{r} - \mathcal{A}_{r - 1} &= \mathcal{E}^{(r)} - \mathcal{E}^{(r - 1)}, \nonumber \\
    &\cdot \nonumber \\
    \mathcal{A}_{r^*} - \mathcal{A}_{r^* - 1} &= \mathcal{E}^{(r^*)} - \mathcal{E}^{(r^* - 1)}.
\end{align}
Moreover, computing the shortest path between nodes $i$ and $j$ on the graph $\mathcal{G}^{(1)}$ can be done as follows. 
\par
If $(i,j) \in \mathcal{E}^{(1)}$, then $d(i,j) = 1$, else if $(i,j) \in \mathcal{E}^{(2)} - \mathcal{E}^{(1)}$, then since $(i,j)$ are $1-$stage neighbors in $\mathcal{G}^{(2)}$ there exists another node $l$ such that $(i, j, l)$ form a triangle in $\mathcal{G}^{(2)}$ and $(i, l), (l, j) \in \mathcal{E}^{(1)}$, hence, $d(i, j) = 2$ in $\mathcal{G}^{(1)}$. Sequentially carrying this one-step computation on the whole sequence $\{ \mathcal{G}^{(r)}\}$ results in 
\begin{equation*}
    d(i, j) = r \mathbb{I}\{(i, j) \in \mathcal{E}^{(r)} - \mathcal{E}^{(r - 1)} \}, 
\end{equation*}
where $\mathbb{I}$ is the indicator function and $\mathcal{E}^{(0)} = \varnothing$, note that these distances correspond to $\mathcal{G}^{(1)}$, and that since all active neighborhood paths remain active if the active length increases by one (i.e., $\mathcal{A}_{r - 1} \subseteq \mathcal{A}_{r}$). By (\ref{eq: second part inverse end}) we have that 
\begin{equation} \label{eq: end first side part b}
    \rho^{(r)} \leq |[\bmat{S}(\omega)]_{ij}| < \rho^{(r - 1)} \implies (i, j) \in \mathcal{A}_r - \mathcal{A}_{r - 1} = \mathcal{P}_{r},
\end{equation}
%which shows the first direction of the second part of Theorem \ref{th: pop_sparsity gnar}.
\end{proof}
\newpage
Furthermore, this shows that defining $\rstage$ neighborhood inclusion based on 
\newline Definition \ref{def: rstage hierarchy} results in the same $\mathcal{A}_{r}$ as defining inclusion based on the underlying network $\mathcal{G}$ under the assumption that larger distance between nodes implies a weaker dependence.
\par
We proceed to prove the other direction of the second part.
\begin{proof}
Consider reparameterizing the process for some $s \leq r^*$ such that $\beta_{kr} \equiv 0$ if and only if $r > s$. 
By Proposition \ref{prop: var constrains} the new linear filters given by (\ref{eq: opt filter}) satisfy that if $(i, j) \notin \mathcal{A}_s,$ then
$$\cov (u_{i, t}^{(ij)|s}, u_{j, t + k}^{(ij)|s}) \equiv 0,$$ 
where $u_{i, t}^{(ij)|s}$ denotes the optimal conditional residuals when restricting the GNAR process to maximum active $\rstage$ depth $s$.
\par
Following the ideas above, for $r \in \{1, \cdots, r^*\}$ restricting the length of $\rstage$ neighborhood regression to a value smaller than $r^*$ results in the optimal filters
\begin{equation*}
     u_{i, t}^{(ij)|r} = X_{i, t} - a_{i} - \sum_{k = 1}^{p} \sum_{l \in \mathcal{A}_r^{(j)}} 
        \gamma_{k}^{il} X_{l, t - k},
\end{equation*}
where $\mathcal{A}_r^{(j)} = \mathcal{A}^{(ij)} \cap \mathcal{A}_r$. And, using Theorem \ref{th: inv spec cross indentity}, (\ref{eq: end first part}, \ref{eq: r stage inv matrix}) we have that
\begin{align} \label{eq: second part end equivalence neigh sets r}
    (i, j ) \in \mathcal{P}_r &\implies (i, j) \in \mathcal{A}_{r}, \nonumber \\
    &\iff |\cov (u_{i, t}^{(ij)|r}, u_{j, t + h}^{(ij)|r} )| \not\equiv 0, \nonumber \\
    &\iff |[\bmat{g}^{(r)} (\omega)]_{ij}| \not\equiv 0. 
\end{align}
\newpage
And, that the reparameterized GNAR process for distances no longer than $(r - 1)$ satisfies
\begin{align} \label{eq: second part end equivalence neigh sets r - 1}
    (i, j) \in \mathcal{P}_{r} &\implies (i, j) \notin \mathcal{A}_{r - 1} \nonumber \\
    &\iff \cov (u_{i, t}^{(ij)|r - 1}, u_{j, t + h}^{(ij)|r - 1}) \equiv 0 \nonumber \\
    &\iff [\bmat{g}^{(r - 1)} (\omega)]_{ij} \equiv 0,
\end{align}
where $\bmat{g}^{(r)} (\omega)$ and $\bmat{g}^{(r - 1)} (\omega)$ are the inverse spectral matrices of the constrained GNAR process. Also note that since
$(i, j) \in \mathcal{A}_{r}$ we have that 
$\bmat{S} (\omega) \not\equiv 0, $
which holds in conjunction with (\ref{eq: second part end equivalence neigh sets r}, \ref{eq: second part end equivalence neigh sets r - 1}). Hence, there exist two threshold values $\rho^{(r)}, \rho^{(r - 1)}$ for each $r \in \{1, \cdots, r^*\}$ in the cross-spectrum hierarchy such that
\begin{align*}
    &\bmat{S}^{(r)}(\omega) = \sft \big( \bmat{S} (\omega) + \rho^{(r)} \diag\{e^{\imath \phi_{ii}}\};  \rho^{(r)} \big) = \bmat{g}^{(r)} (\omega), \\
     &\bmat{S}^{(r - 1)}(\omega) = \sft \big( \bmat{S} (\omega) + \rho^{(r - 1)} \diag\{e^{\imath \phi_{ii}}\};  \rho^{(r - 1)} \big) = \bmat{g}^{(r - 1)} (\omega),
\end{align*}
which gives $\rho^{(r)} \leq |[\bmat{S}(\omega)]_{ij}| < \rho^{(r - 1)}$, and we have that
\begin{equation} \label{eq: end second side b}
    (i, j) \in \mathcal{P}_{r} \implies \rho^{(r)} \leq |[\bmat{S}(\omega)]_{ij}| < \rho^{(r - 1)},
\end{equation}
for all $\omega \in [-\pi, \pi]$.
\end{proof}
%Proof ends here
Finally, combining (\ref{eq: end first side part b}, \ref{eq: end second side b}) and Proposition \ref{prop: distance for conditional independence} finishes the proof.
\par
The ideas in this proof show how stronger dependence between closer nodes can be exhibited either by pruning the latent graph $\tilde{\mathcal{G}}$ or by applying the soft-threshold given by (\ref{eq: cmplx sft}) to $\bmat{S} (\omega)$ (i.e., a form of reparameterization), which are equivalent. Furthermore, they establish the equivalence between using the generalized GNAR correlation structure $\mathcal{G}$ and the notions of different degrees of dependence in Definitions \ref{def: conditional indep definition} and \ref{def: rstage hierarchy} with the notions in Section \ref{sec:gnar methodology}.
\newpage
\begin{remark} \label{rma: graph generalization}
Let $\mathcal{G}^{(1)} = (\mathcal{K}, \mathcal{E}^{(1)})$ be the graph associated to the strongest connections with edge set $\mathcal{E}^{(1)}$ given by (\ref{eq: r sequence equivalence}), then the graph $G = (\mathcal{K}, E)$ given by Definition \ref{def: conditional indep definition} is the same graph (i.e., $\mathcal{G}^{(1)} = G$).
\end{remark}

Remark \ref{rma: graph generalization} shows how GNAR processes generalize graphical multivariate time series by constraining VAR models with the introduction of higher-order interactions, furthermore, it shows that the neighborhood regression coefficients $\beta_{kr}$ exploit the correlation structure induced by $\mathcal{G}$ since they account for node-wise interactions common across the network and manage inclusion in active $\rstage$ conditional dependence paths.
\begin{corollary} \label{cor: simplify to graphical models}
If one constrains a stationary $\GNAR(p, [s_1, \cdots, s_p])$ $\boldsymbol{X}_t$ process to $1-$stage neighborhood regression, then the correlation hierarchy in Definition \ref{def: rstage hierarchy} simplifies to only distinguishing between $[\bmat{S} (\omega)]_{ij} \equiv 0$ and $[\bmat{S} (\omega)]_{ij} \not\equiv 0$, hence, Theorem \ref{th: pop_sparsity gnar} recovers the results in \cite{graph_series}.
\end{corollary}
Corollary \ref{cor: simplify to graphical models} shows that $\GNAR(p, [1, \cdots, 1])$ is equivalent to parsimonious partial correlation graphical models that satisfy the Markov properties of graphical models; see \cite{graph_series} and \cite{lauritzen}.



